LG-FiLM: Local-Global Mixture-of-Experts Modulation for RAW-to-RGB Reconstruction

An image signal processor does more than reconstruct an image. It also has to decide how strongly to denoise, how to balance color, and which tone curve maps the scene onto the display, and these settings depend on the scene itself, the curve that suits a backlit sky is not the one that suits an indoor portrait. Most neural ISPs learn a single fixed transformation and apply it to every scene. We instead make the adaptation an explicit part of the network. Our model, LG FiLM, keeps one shared encoder decoder and places a small mixture of affine experts at its bottleneck; the experts scales, shifts, and mixing weights are predicted from local neighborhood evidence together with a global scene descriptor. Reconstruction stays in a single shared pathway and only the processing mode is switched. We evaluate LG FiLM on three datasets, Fujifilm UltraISP, Zurich RAW to RGB, and a COCO derived benchmark built with an inverse ISP. The model reaches the best reconstruction fidelity of the compared entries on the primary benchmark and transfers to the other two.

==> LG-FiLM_RAW-to-RGB/architecture.tex <==
% 方法结构示意图，由当前模型数据流绘制，不是定性实验图。
\begin{figure}[t]
\centering
\definecolor{lgink}{HTML}{26354A}
\definecolor{lgpanel}{HTML}{F8FAFC}
\definecolor{lgborder}{HTML}{CBD5E1}
\definecolor{lgblue}{HTML}{427BB8}
\definecolor{lgteal}{HTML}{258C84}
\definecolor{lgviolet}{HTML}{8062AB}
\definecolor{lgorange}{HTML}{CE8630}
\definecolor{lgrose}{HTML}{BD627E}
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
  font=\sffamily\fontsize{8}{9.5}\selectfont,text=lgink,
  block/.style={rounded corners=2pt,line width=0.65pt,align=center,
    minimum height=0.78cm,inner sep=3pt},
  encoder/.style={block,draw=lgblue,fill=lgblue!12,text width=1.20cm},
  decoder/.style={block,draw=lgteal,fill=lgteal!12,text width=1.20cm},
  flow/.style={-{Latex[length=1.6mm,width=1.1mm]},draw=lgink,line width=0.75pt},
  skip/.style={flow,draw=lgteal,dashed,rounded corners=2pt},
  weight/.style={flow,draw=lgviolet,dashed,rounded corners=2pt},
  title/.style={font=\sffamily\bfseries\fontsize{10}{11}\selectfont,anchor=west},
  note/.style={font=\sffamily\fontsize{7}{8}\selectfont,align=center},
  port/.style={circle,draw=lgteal,fill=white,inner sep=0pt,
    minimum size=0.23cm,font=\sffamily\fontsize{8}{8}\selectfont}]
% 两个同宽浅色面板兼作独立图片导出的矢量边界。
\draw[draw=lgborder,fill=lgpanel,rounded corners=4pt,line width=0.6pt]
  (0,4.18) rectangle (19,7.95);
\draw[draw=lgborder,fill=lgpanel,rounded corners=4pt,line width=0.6pt]
  (0,0) rectangle (19,3.86);
\node[title] at (0.30,7.66) {(a) Network architecture};
\node[anchor=east,font=\sffamily\bfseries\fontsize{8}{9}\selectfont,
  text=lgorange] at (18.68,7.66) {Default configuration: 8 experts};
\node[note,text=lgblue] at (3.8,7.33) {SHARED ENCODER};
\node[note,text=lgteal] at (15.1,7.33) {SHARED DECODER};
\node[note,text=lgteal] at (9.5,7.33) {$\oplus$ Additive skip connections};
% 输入 Bayer 图案和输出三通道卡片均为示意符号，不是实验图像。
\foreach \i in {0,...,3} {
  \foreach \j in {0,...,3} {
    \pgfmathtruncatemacro{\bayercell}{mod(\i,2)+2*mod(\j,2)}
    \ifcase\bayercell\def\cellcolor{lgteal}\or\def\cellcolor{lgblue}%
      \or\def\cellcolor{lgrose}\or\def\cellcolor{lgteal}\fi
    \fill[\cellcolor!65,draw=white,line width=0.3pt]
      (0.28+\i*0.19,6.20+\j*0.19) rectangle ++(0.19,0.19);
  }
}
\node[note,font=\sffamily\fontsize{6.3}{8}\selectfont] at (0.66,5.90)
  {Sparse RAW\\$3,\;H$};
\coordinate (rawout) at (1.06,6.58);
\node[encoder,text width=1.08cm] (stem) at (2.05,6.58)
  {\textbf{Stem}\\$16,\;H$};
\node[encoder] (enc1) at (3.90,6.32) {\textbf{Enc. 1}\\$32,\;H/2$};
\node[encoder] (enc2) at (5.50,5.78) {\textbf{Enc. 2}\\$64,\;H/4$};
\node[encoder] (enc3) at (7.10,5.24) {\textbf{Enc. 3}\\$128,\;H/8$};
\node[block,draw=lgorange,fill=lgorange!17,line width=1pt,
  text width=2.30cm,minimum height=0.92cm] (bottleneck) at (9.50,5.24)
  {\textbf{LG-FiLM}\\$128\!\rightarrow\!256,\;H/8$\\[-1pt]
   {\fontsize{7}{8}\selectfont 8 affine experts}};
\node[decoder] (dec3) at (11.90,5.24) {\textbf{Dec. 3}\\$128,\;H/8$};
\node[decoder] (dec2) at (13.50,5.78) {\textbf{Dec. 2}\\$64,\;H/4$};
\node[decoder] (dec1) at (15.10,6.32) {\textbf{Dec. 1}\\$32,\;H/2$};
\node[block,draw=lgrose,fill=lgrose!12,text width=1.12cm] (head) at (16.90,6.58)
  {\textbf{Head}\\PS$\times2$};
\fill[lgblue!65,draw=white] (17.99,6.29) rectangle (18.55,6.89);
\fill[lgteal!65,draw=white] (18.10,6.20) rectangle (18.66,6.80);
\fill[lgrose!65,draw=white] (18.21,6.11) rectangle (18.77,6.71);
\node[note] at (18.38,5.90) {RGB\\$3,\;H$};
\draw[flow] (rawout)--(stem.west);
\foreach \a/\b in {stem/enc1,enc1/enc2,enc2/enc3,enc3/bottleneck,
  bottleneck/dec3,dec3/dec2,dec2/dec1,dec1/head} {
  \draw[flow] (\a.east)--(\b.west);
}
\draw[flow] (head.east)--(17.97,6.58);
\foreach \n/\height in {1/7.02,2/6.48,3/5.94} {
  \node[port] (add\n) at (dec\n.center |- 0,\height) {$+$};
  \draw[skip] (enc\n.north)--(enc\n.center |- 0,\height)
    --(add\n.west);
  \draw[draw=lgteal,line width=0.75pt] (add\n.south)--(dec\n.north);
}
\node[note,anchor=west] at (0.32,4.47)
  {Encoder: stride-2 Conv + 2 RBs\quad Decoder: Conv + resize + $\oplus$ + RB};
\node[note,anchor=east] at (18.68,4.47)
  {RB: residual block\quad Head: Conv + PS$\times2$ + ReLU};
\draw[draw=lgorange,dashed,line width=0.8pt]
  (bottleneck.south)--(9.50,4.64);
\draw[flow,draw=lgorange,dashed] (9.50,4.16)--(9.50,3.88);
% 瓶颈放大图：同一局部—全局条件同时进入路由器和全部专家。
\node[title] at (0.30,3.57) {(b) LG-FiLM bottleneck};
\node[note,anchor=east] at (18.68,3.57)
  {$H=W=256:\quad h=w=32,\quad C=128,\quad N=1{,}024$ tokens};
\node[block,draw=lgblue,fill=lgblue!9,text width=0.73cm,
  minimum height=0.68cm] (feature) at (0.62,1.94) {$\feat_{\rm enc}$\\$128$};
\node[encoder,text width=1.08cm,minimum height=0.68cm] (shared) at (2.04,1.94)
  {Shared\\RBs $\times2$};
\coordinate (f) at (3.03,1.94);
\fill[lgink] (f) circle (1.2pt);
\node[above right=1pt] at (f) {$\feat$};
\node[block,draw=lgteal,fill=lgteal!12,text width=1.48cm] (local) at (4.50,2.62)
  {\textbf{Local}\\{\fontsize{7}{8}\selectfont $3\!\times\!3$ DWConv}};
\node[block,draw=lgviolet,fill=lgviolet!12,text width=1.48cm] (global) at (4.50,1.18)
  {\textbf{Global}\\{\fontsize{6.7}{8}\selectfont GAP + broadcast}};
\node[block,draw=lgviolet,fill=lgviolet!7,text width=1.48cm] (concat) at (6.64,1.94)
  {\textbf{Concat}\\$\ctx_i=[\mathbf u_i;\mathbf g]$};
\node[block,draw=lgviolet,fill=lgviolet!15,text width=2.15cm] (router) at (9.02,2.68)
  {\textbf{Router}\\{\fontsize{7}{8}\selectfont Linear + softmax}\\$p_{i,1},\ldots,p_{i,8}$};
\node[block,draw=lgorange,fill=lgorange!6,text width=2.62cm,
  minimum height=1.55cm,inner sep=0pt] (experts) at (9.02,1.13) {};
\node[note,font=\sffamily\bfseries\fontsize{8}{9}\selectfont] at (9.02,1.65)
  {8 affine experts};
\foreach \k/\x/\y in {1/8.10/1.27,2/8.71/1.27,3/9.32/1.27,4/9.93/1.27,
                        5/8.10/0.86,6/8.71/0.86,7/9.32/0.86,8/9.93/0.86} {
  \node[draw=lgorange!75,fill=lgorange!18,rounded corners=1pt,
    minimum width=0.47cm,minimum height=0.30cm,inner sep=1pt,note] at (\x,\y) {$e_{\k}$};
}
\node[note] at (9.02,0.51) {MLP $\rightarrow(\gamma_{i,k},\beta_{i,k})$};
\node[block,draw=lgorange,fill=lgorange!13,text width=2.22cm,
  minimum height=1.02cm] (fusion) at (12.02,1.94)
  {\textbf{Soft fusion}\\
   $\bar\gamma_i=\sum_k p_{i,k}\gamma_{i,k}$\\
   $\bar\beta_i=\sum_k p_{i,k}\beta_{i,k}$};
\node[block,draw=lgrose,fill=lgrose!12,text width=2.24cm,
  minimum height=1.02cm] (affine) at (15.02,1.94)
  {\textbf{Modulation}\\
   $\feat_i'=\feat_i\odot(1+\bar\gamma_i)$\\$+\;\bar\beta_i$};
\node[block,draw=lgblue,fill=lgblue!12,text width=1.25cm,
  font=\sffamily\fontsize{7}{8}\selectfont] (projection) at (17.37,1.94)
  {$1\!\times\!1$ Conv\\$128\!\rightarrow\!256$};
\draw[flow] (feature)--(shared);
\draw[draw=lgink,line width=0.75pt] (shared.east)--(f);
\draw[flow] (f)|-(local.west);
\draw[flow] (f)|-(global.west);
\draw[flow,draw=lgteal] (local.east)-|(concat.north);
\draw[flow,draw=lgviolet] (global.east)-|(concat.south);
\coordinate (condition) at (7.63,1.94);
\draw[draw=lgink,line width=0.75pt] (concat.east)--(condition);
\draw[flow] (condition)|-(router.west);
\draw[flow] (condition)|-(experts.west);
\draw[weight] (router.east)-|(fusion.north);
\draw[flow,draw=lgorange] (experts.east)-|(fusion.south);
\draw[flow,draw=lgorange] (fusion)--(affine);
\draw[flow] (affine)--(projection);
\draw[flow] (projection.east)--(18.57,1.94);
\node[note] at (18.51,1.48) {$\feat_{\rm out}$};
\draw[flow,rounded corners=2pt] (f)--(3.03,0.19)--(15.02,0.19)--(affine.south);
\node[note,fill=lgpanel,inner sep=2pt] at (12.40,0.19) {Shared feature $\feat_i$};
\node[note,text=lgorange] at (12.02,0.91) {All experts, every token};
\node[note,text=lgviolet] at (6.64,0.92) {$\ctx_i\in\mathbb R^{2C}$};
\end{tikzpicture}}
\caption{Architecture of \method. (a) Sparse three-channel RAW preserves sensor-grid alignment through a shared encoder--decoder with three additive skips. Stage labels give channels and height; width scales identically. The deepest decoder stage preserves resolution. (b) Local and global context jointly condition softmax attention over eight affine experts and their transformations. Soft fusion mixes scale and shift parameters to modulate the shared feature before projection. Expert output heads are zero-initialized.}
\label{fig:architecture}
\end{figure}


==> LG-FiLM_RAW-to-RGB/coco_figure.tex <==
% COCO 验证集预测/GT 对照，四张图由 test.py 在同一 checkpoint 上重跑生成。
% 行标签由 \caption 说明（Top row / bottom row），图下不再重复标注。
\begin{figure}[t]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}cccc@{}}
\includegraphics[width=0.23\textwidth]{000000110359_pred.jpg} &
\includegraphics[width=0.23\textwidth]{000000491757_pred.jpg} &
\includegraphics[width=0.23\textwidth]{000000349837_pred.jpg} &
\includegraphics[width=0.23\textwidth]{000000380711_pred.jpg} \\[2pt]
\includegraphics[width=0.23\textwidth]{000000110359_gt.jpg} &
\includegraphics[width=0.23\textwidth]{000000491757_gt.jpg} &
\includegraphics[width=0.23\textwidth]{000000349837_gt.jpg} &
\includegraphics[width=0.23\textwidth]{000000380711_gt.jpg} \\
\end{tabular}
\caption{Reconstruction examples on the InvISP-derived COCO test set. Top row: \method{} outputs; bottom row: the COCO references.}
\label{fig:coco}
\end{figure}


==> LG-FiLM_RAW-to-RGB/mechanism_figures.tex <==
% 由冻结模型的实际路由、专家移除对照和 GT 生成，无合成热图。
% 主文只保留核心干预对照（bypass / fixed prior / learned mixture）；
% 单个专家贡献图已移至 supplement.tex（fig:mechanism_routing，S2）。
\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{mechanism_comparison.pdf}
\caption{Effect of expert modulation and adaptive routing. Three selected official-validation scenes compare GT, bypassed modulation, a fixed routing prior, and the learned mixture. The prior fixes mean weights across inputs and locations but retains input-conditioned expert transformations. RGB panels share a display range; absolute luminance errors share $[0,0.15]$, with larger values saturating.}
\label{fig:mechanism_comparison}
\end{figure}


==> LG-FiLM_RAW-to-RGB/mechanism_table.tex <==
% 由 render_mechanism.py 按独立冻结推理记录生成。
\begin{table}[t]
\centering\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lrr}
\toprule
Inference intervention & RGB PSNR & Y-MAE \\
\midrule
Modulation bypassed & 20.073 & 0.07365 \\
Uniform weights & 21.588 & 0.08544 \\
Permuted expert weights & 20.574 & 0.09667 \\
Fixed routing prior & 24.463 & 0.05434 \\
Token-hard argmax & 24.367 & 0.05177 \\
Image-mean weights & 24.972 & 0.04919 \\
Spatially shuffled weights & 24.968 & 0.04920 \\
\method & 24.997 & 0.04914 \\
\bottomrule
\end{tabular}
\caption{Modulation and routing interventions on the test set. The permuted row averages seven nonidentity cyclic permutations of the expert-weight assignments.}
\label{tab:mechanism}
\end{table}


==> LG-FiLM_RAW-to-RGB/qualitative_figure.tex <==
% 由 prepare_evidence.py 从已保存的测试输出生成，图像像素保持不变。
% 行标签由 \caption 说明，图下不再重复标注；六张图铺满整行宽度。
\begin{figure}[t]
\centering
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{@{}cccccc@{}}
\includegraphics[width=0.155\textwidth]{1585_pred.png} &
\includegraphics[width=0.155\textwidth]{313_pred.png} &
\includegraphics[width=0.155\textwidth]{257_pred.png} &
\includegraphics[width=0.155\textwidth]{2034_pred.png} &
\includegraphics[width=0.155\textwidth]{2173_pred.png} &
\includegraphics[width=0.155\textwidth]{746_pred.png} \\[2pt]
\includegraphics[width=0.155\textwidth]{1585_gt.png} &
\includegraphics[width=0.155\textwidth]{313_gt.png} &
\includegraphics[width=0.155\textwidth]{257_gt.png} &
\includegraphics[width=0.155\textwidth]{2034_gt.png} &
\includegraphics[width=0.155\textwidth]{2173_gt.png} &
\includegraphics[width=0.155\textwidth]{746_gt.png} \\[2pt]
\end{tabular}
\caption{Qualitative comparison across varied scenes. Top row: \method{} outputs; bottom row: corresponding ground truth. Every panel shows the complete evaluation patch.}
\label{fig:qualitative}
\end{figure}


==> LG-FiLM_RAW-to-RGB/results_figure.tex <==
% 对照两个本地评测集合的 PSNR/SSIM；不把外部挑战赛拼成同协议曲线。
\begin{figure}[t]
\centering
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[width=\linewidth,height=4.8cm,
 ylabel={RGB PSNR (dB)},
 symbolic x coords={Linear,Cosine,Additive,LG-FiLM,Expanded},xtick=data,
 xticklabel style={font=\scriptsize},
 ymin=24.4,ymax=26.05,grid=major,grid style={gray!20},
 tick label style={font=\small},label style={font=\small},
 legend style={font=\scriptsize,at={(0.5,1.02)},anchor=south,legend columns=2},
 enlarge x limits=0.12]
\addplot[color=plotblue,mark=square*,thick,dashed] coordinates {
 (Linear,25.313) (Cosine,24.927) (Additive,25.685) (LG-FiLM,25.758) (Expanded,25.864)};
\addlegendentry{Val}
\addplot[color=plotgreen,mark=*,thick] coordinates {
 (Linear,24.652) (Cosine,24.912) (Additive,24.737) (LG-FiLM,24.998) (Expanded,24.891)};
\addlegendentry{Test}
\end{axis}
\end{tikzpicture}
\caption{PSNR ordering differs between the Val and Test sets.}
\end{subfigure}\hfill
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[width=\linewidth,height=4.8cm,
 ylabel={SSIM},
 symbolic x coords={Linear,Cosine,Additive,LG-FiLM,Expanded},xtick=data,
 xticklabel style={font=\scriptsize},
 ymin=0.878,ymax=0.890,grid=major,grid style={gray!20},
 scaled y ticks=false,yticklabel style={/pgf/number format/fixed,/pgf/number format/precision=3},
 tick label style={font=\small},label style={font=\small},
 legend style={font=\scriptsize,at={(0.5,1.02)},anchor=south,legend columns=2},
 enlarge x limits=0.12]
\addplot[color=plotblue,mark=square*,thick,dashed] coordinates {
 (Linear,0.88407) (Cosine,0.88617) (Additive,0.88776) (LG-FiLM,0.88761) (Expanded,0.88820)};
\addlegendentry{Val}
\addplot[color=plotgreen,mark=*,thick] coordinates {
 (Linear,0.88050) (Cosine,0.88456) (Additive,0.88206) (LG-FiLM,0.88366) (Expanded,0.88272)};
\addlegendentry{Test}
\end{axis}
\end{tikzpicture}
\caption{SSIM ordering differs from PSNR.}
\end{subfigure}
\caption{Local quality on the Val and Test sets. Linear/Cosine denote image-level routers, Additive denotes local--global additive experts, and Expanded denotes the conditioned 16-expert variant. Expanded improves Val but falls below \method{} on Test.}
\label{fig:results}
\end{figure}


==> mechanism_figures.tex <==
% 由冻结模型的实际路由、专家移除对照和 GT 生成，无合成热图。
% 主文只保留核心干预对照（bypass / fixed prior / learned mixture）；
% 单个专家贡献图已移至 supplement.tex（fig:mechanism_routing，S2）。
\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{mechanism_comparison.pdf}
\caption{Effect of expert modulation and adaptive routing. Three selected official-validation scenes compare GT, bypassed modulation, a fixed routing prior, and the learned mixture. The prior fixes mean weights across inputs and locations but retains input-conditioned expert transformations. RGB panels share a display range; absolute luminance errors share $[0,0.15]$, with larger values saturating.}
\label{fig:mechanism_comparison}
\end{figure}


==> qualitative_figure.tex <==
% 由 prepare_evidence.py 从已保存的测试输出生成，图像像素保持不变。
% 行标签由 \caption 说明，图下不再重复标注；六张图铺满整行宽度。
\begin{figure}[t]
\centering
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{@{}cccccc@{}}
\includegraphics[width=0.155\textwidth]{1585_pred.png} &
\includegraphics[width=0.155\textwidth]{313_pred.png} &
\includegraphics[width=0.155\textwidth]{257_pred.png} &
\includegraphics[width=0.155\textwidth]{2034_pred.png} &
\includegraphics[width=0.155\textwidth]{2173_pred.png} &
\includegraphics[width=0.155\textwidth]{746_pred.png} \\[2pt]
\includegraphics[width=0.155\textwidth]{1585_gt.png} &
\includegraphics[width=0.155\textwidth]{313_gt.png} &
\includegraphics[width=0.155\textwidth]{257_gt.png} &
\includegraphics[width=0.155\textwidth]{2034_gt.png} &
\includegraphics[width=0.155\textwidth]{2173_gt.png} &
\includegraphics[width=0.155\textwidth]{746_gt.png} \\[2pt]
\end{tabular}
\caption{Qualitative comparison across varied scenes. Top row: \method{} outputs; bottom row: corresponding ground truth. Every panel shows the complete evaluation patch.}
\label{fig:qualitative}
\end{figure}

